EFloat: Entropy-coded Floating Point Format for Compressing Vector Embedding Models

In a large class of deep learning models, including vector embedding models such as word and database embeddings, we observe that floating point exponent values cluster around a few unique values, permitting entropy based data compression. Entropy coding compresses fixed-length values with variable-length codes, encoding most probable values with fewer bits. We propose the EFloat compressed floating point number format that uses a variable field boundary between the exponent and significand fields. EFloat uses entropy coding on exponent values and signs to minimize the average width of the exponent and sign fields, while preserving the original FP32 exponent range unchanged. Saved bits become part of the significand field increasing the EFloat numeric precision by 4.3 bits on average compared to other reduced-precision floating point formats. EFloat makes 8-bit and even smaller floats practical without sacrificing the exponent range of a 32-bit floating point representation. We currently use the EFloat format for saving memory capacity and bandwidth consumption of large vector embedding models such as those used for database embeddings. Using the RMS error as metric, we demonstrate that EFloat provides higher accuracy than other floating point formats with equal bit budget. The EF12 format with 12-bit budget has less end-to-end application error than the 16-bit BFloat16. EF16 with 16-bit budget has an RMS-error 17 to 35 times less than BF16 RMS-error for a diverse set of embedding models. When making similarity and dissimilarity queries, using the NDCG ranking metric, EFloat matches the result quality of prior floating point representations with larger bit budgets.

==> hardware.tex <==

Hardware arithmetic functional units natively supporting EFloat operations currently do not
exist.  To/from conversion existing floating point(FP) to EFloat (EF) format will be necessary before/after operating on
the floats.  EF support will be different depending on the whether the
accelerator is used for {\em inferencing} or {\em training}.  For
inferencing, the trained AI models may be converted to the EF format
once and placed in the system or accelerator memory in read-only
form. FP to EF conversion may be done in software; no EF encoding
hardware is necessary since this step is not time critical.
However, EF decoding hardware will be necessary before feeding the
EF-coded model weights to the functional units.  EF decoders may be
placed anywhere between the memory and the functional unit.  If the
accelerator is bandwidth limited then EF decoders may be placed before
the accelerator inputs or next to the accelerator side of the
communication links, i.e., memory bus, chip fabric, or PCIe links.

EF decoding hardware may be implemented with a SRAM lookup table.
With a maximum code width of $K$ bits a $2^K$ entry SRAM based table
may be used. $K=8$ is desirable to cover the worst case condition of
all 256 exponents utilized by an FP32 dataset.
The table is indexed by the coded-exponent. Each entry consists of
the original exponent and the coded-exponent's bit-width.
As stated in Section~\ref{sec:impl} many entries in
the lookup table will be filled with duplicates for decoding
shorter than maximum width coded-exponents.

When the accelerator has many input ports, for example a systolic
array such as the Google TPU~\cite{jouppi2018motivation}, or a wide SIMD architecture~\cite{henry2020high,hennessy2017computer}, many decoder tables will be necessary for
parallel access.  To save area, the maximum code width may be set to
$K < 8$ at the expense of giving up some compression quality.  An
alternative approach for saving area might be using a two level table
which will substantially reduce SRAM capacity requirements.
First level table is indexed by the most significant bits of the code
and the second level table is indexed by the least significant bits of the code.
Huffman prefix-trees have the property that the leading bits of
infrequent codes are
substantially identical which results in many shared entries
in the first level table.  For example, the Zlib
software~\cite{zlib:library} employing Huffman codes uses a maximum code width of 15-bits.  But
for encoding of 512 Zlib symbols, a 2-level table needs only 852
table entries compared to $2^{15}=32768$ entries required in a 1-level table.
% put this link in the citation https://github.com/madler/zlib/blob/master/inftrees.h#L38

For training, the accelerator will perform many weight updates,
writing floats back to the memory during training iterations.
Therefore EF encoders must be placed at the accelerator outputs. EF
encoding hardware may be implemented with an SRAM lookup table indexed
with the original exponent.  Each table entry consists of a
coded-exponent and its bit width.

Functional units natively processing EF floats do not exist
yet. Therefore, an EF float must be first converted to a plain unencoded
float. FP multipliers and adders must be sized to accommodate the
maximum possible mantissa width. For example, BF16 has an 8-bit
exponent and 7-bit mantissa. EF16 with minimum 2-bit coded-exponent
also has an 8-bit exponent but a 13-bit mantissa which will result
in a larger EF16 multiplier than for BF16.  To have similar area, 
one might consider using a smaller EF10 format instead of EF16.


==> signi.tex <==
Figures~\ref{fig:benford} and ~\ref{fig:bit-distr} present patterns observed in the significands of FP32 values of 
various pre-trained vector embedding models used in the evaluation of EFloat format. Figure~\ref{fig:benford} plots the frequency 
distribution of the most significant significand digit in the decimal representation of the FP32 values. Occurrences of
these digits follow a logarithmically decreasing distribution, called Benford's law~(\citet{newcomb-law, benford-law}). According to Benford's Law,
the number 1 occurs as the most significant digit about 30.1\% of time, number 2 17.6\% of time, and so on. The logarithmic reduction
leads to the number 9 being at the most significant location around 4.6\% of time.

\begin{figure}[ht]
  \centering
  %left lower right upper
  \includegraphics[width=0.48\textwidth]{../benford.png}
  %\vskip -0.05in
  \caption{The most significant decimal digit in the significand of FP32 values in various vector embedding models follows the Benford distribution.}
  \label{fig:benford}
  %\vskip -0.1in
\end{figure}

Figure~\ref{fig:bit-distr} presents a bit-specific view of the same datasets. 
In this Figure, we report the agregate distribution of a particular bit location having the value 1 for 23 
significand bits computed over all FP32 entries of the selected vector embedding models. As we observe, the distribution exhibits 
a knee at location 7; the first 7 bits show an increase in the probability of the bit value being 1 from 41.51\% to 49.88\%; 
the remaining bits exhibit probabilities around 50\%. In other words, it is more likely to see bit values being 0 in the most significant bit locations
of FP32 values in the pre-trained vector embedding models.

\begin{figure}[ht]
  \centering
  %left lower right upper
  \includegraphics[width=0.48\textwidth]{../bit-distr.png}
  %\vskip -0.05in
  \caption{Distribution of a bit value being 1 at different bit locations in the significand of FP32 values in various vector embedding models.}
  \label{fig:bit-distr}
  %\vskip -0.1in
\end{figure}




